A Kernel-Based View of Language Model Fine-Tuning

It has become standard to solve NLP tasks by fine-tuning pre-trained language models (LMs), especially in low-data settings. There is minimal theoretical understanding of empirical success, e.g., why fine-tuning a model with $10^8$ or more parameters on a couple dozen training points does not result in overfitting. We investigate whether the Neural Tangent Kernel (NTK) - which originated as a model to study the gradient descent dynamics of infinitely wide networks with suitable random initialization - describes fine-tuning of pre-trained LMs. This study was inspired by the decent performance of NTK for computer vision tasks (Wei et al., 2022). We extend the NTK formalism to Adam and use Tensor Programs (Yang, 2020) to characterize conditions under which the NTK lens may describe fine-tuning updates to pre-trained language models. Extensive experiments on 14 NLP tasks validate our theory and show that formulating the downstream task as a masked word prediction problem through prompting often induces kernel-based dynamics during fine-tuning. Finally, we use this kernel view to propose an explanation for the success of parameter-efficient subspace-based fine-tuning methods.

==> acknowledgements.tex <==
\section*{Acknowledgements}
We thank Tianyu Gao, Wei Hu, Jason Lee, Kaifeng Lyu, Abhishek Panigrahi, Nikunj Saunshi, Mengzhou Xia, and Greg Yang for their helpful comments and discussion.
This work is funded by NSF, ONR, Simons Foundation, DARPA and SRC. 

==> kernel_notes.tex <==

\section{Notes on Kernel}\label{sec:kernel_computation}
The NTK takes an initialization of a network (in this case, the pre-trained network) and models what the trained network would output. We cannot directly model what the trained network's parameters are -- we can only simulate what the trained network will do.

\subsection{Computing the Kernel}
Let $f:\gS\to\sR^C$ be the downstream-task-aware transformer function, where $\gS$ is the set of all possible contexts (with a prompt included), and the output of the transformer is the logit vector of the words corresponding to the $C$ classes in the problem. For example, for SST-2, $f$ takes in ``$\langle S_1\rangle$ It was [MASK] .'' where $\langle S_1\rangle$ is the movie review. Then, $f$ outputs a 2-dimensional vector with the logit assigned to ``great'' and the logit assigned to ``terrible'' filling in the [MASK] token. 

The NTK formulation says that we can model what the transformer would output for these logits after fine-tuning. To compute the NTK, we need to take the following steps:
\begin{enumerate}
	\item Decide if we are modeling across logits or modeling each logit individually. See \Cref{sec:logit_model}.
	\item Select a kernel formula: SGD, SignGD, or Asymmetric SignGD. See \Cref{sec:kernel_formula}.
	\item Compute the train-train kernel using the kernel formula. If modeling across logits, it will be $1\times CK \times CK$. If modeling logits individually, it will be $C\times K\times K$. In the special case of modeling logits individually for binary classification, the kernel will be $1\times K\times K$, since modeling one logit is sufficient.
	\item Solve for the coefficients $\alpha$. See \Cref{sec:kernel_solvers}.
	\item Compute the train-validation and train-test kernels using the same kernel formula. The first dimension will depend on the logit modeling, the second will be the train set size $K$, and the third will be the size of the validation or test set accordingly. For the few-shot setting, the train-test kernel is the most expensive to compute.
\end{enumerate}

\subsection{Modeling Logits}\label{sec:logit_model}
We can either model across logits or model each logit individually. $f$ outputs $C$ values for the logits. We use $g_i(c)$ to denote the gradient of the network output for the word corresponding to class $c$ when given datapoint $i$ as input. $g_i(c)$ is a flattened vector of the gradient wrt all parameters that are trained during fine-tuning. The standard (SGD) kernel formula is $\langle g_i(c), g_j(c)\rangle$, and we use this formula to illustrate the different logit modeling techniques here. We will also focus on the square train-train kernel for ease of presentation.

\textbf{Modeling each logit individually} means that the outputs of the network for different classes are treated as independent outputs. We construct and solve $C$ distinct kernel regression problems to model the $C$ outputs. Hence, the kernel can be thought of as $C\times K \times K$, or just $C$ different $K\times K$ kernels. Each kernel will fix $c$ and compute $\gK(i,j) = \langle g_i(c), g_j(c)\rangle$.

The benefit is that the computation only scales linearly with the number of classes. The downside is that the network loses the chance to rank classes against each other and instead has to model the likelihoods of each class individually. The difficulty of this independent modeling scales with the number of classes there are. 

\textbf{Modeling across logits} means that the network models interactions across logits for each datapoint. Each datapoint generates $C$ outputs, so we actually have $CK$ gradients to compute. We can think of this as augmenting our dataset size by a factor of $C$. Now the kernel function takes in two classes to compare in addition to two datapoints to compare: $\gK(c_i, c_j, i, j)=\langle g_i(c_i), g_j(c_j)\rangle$. In implementation, we still model the kernel as a two-dimensional $CK\times CK$ matrix but note that it has some special structure within it.

Suppose we fix $c_i=c_j$. This recovers the case above, where we model each logit individually. We would take dot products comparing the representations of datapoints $i$ and $j$ in an effort to model the logit $c_i=c_j=c$. 

Suppose we fix $i=j$ and $c_i\neq c_j$. Now we are performing a computation we never did in the previous case: we are comparing the values of different logits across classes \textbf{for the same datapoint}. We are actually allowing the network to compare logits on ``great'' and ``terrible'' in order to model the logit for ``great''. 

\textbf{Special Case: Binary Classification} In the case of binary classification, we actually only need to model one logit in order to model the other one. So, if we are modeling logits individually, we can just model the positive logit and take its complement to recover the negative one. Note that we only see the benefit of modeling across logits if we model the two logits separately. Also, for binary classification, we found the output that works best is positive logit - negative logit, so we use this as the single output of the network function $f$ to model.

\subsection{Kernel Formulas}\label{sec:kernel_formula}
There are different kernel formulas $\gK$ that can be used. Each formula corresponds to a different training (ie fine-tuning) optimization algorithm. All of them operate on the gradient on an individual datapoint. We will focus on the general case of modeling across logits to illustrate the formulas (see previous section for logit modeling discussion).
\begin{enumerate}
	\item \textbf{SGD}: $\gK(c_i, c_j,i,j) = \langle g_i(c_i), g_j(c_j)\rangle$
	\item \textbf{SignGD}: $\gK(c_i, c_j, i, j) = \langle \sgn(g_i(c_i)), \sgn(g_j(c_j))\rangle$
	\item \textbf{Asymmetric SignGD}: $\gK(c_i, c_j, i, j) = \langle g_i(c_i), \sgn(g_j(c_j))\rangle$
\end{enumerate}

Here, the $\sgn$ operator indicates taking the element-wise sign function of the gradient vector (ie turning each entry into $\pm 1$). 

\paragraph{SGD} The SGD formula is the only existing one in literature so far. It models fine-tuning with SGD (or GD). When people say NTK nowadays, they mean this formula.

\paragraph{SignGD} The SignGD formula arises through some hand-wavy reasoning. The idea is that Adam behaves similar to SignGD in the very early stages, because the second order moment and the momentum have not gotten any information yet and thus just provide naive element-wise normalization to the gradient. You can see this discussed between Propositions 2 and 3 in \cite{ma2020qualitative}. Replacing the gradients in the SGD formula with their sign immediately yields the formula.

\paragraph{Asymmetric SignGD} The Asymmetric SignGD formula is one of the theoretically correct limits for Adam. When considering a limit for Adam, one needs to carefully choose how quickly to take the learning rate to a limit in relation to taking the momentum averaging hyperparameters to their limits. You can see this in Section 2.2 in \cite{ma2020qualitative}. One limit (likely the only one we can compute) gives us this asymmetric kernel formula. The rigorous derivation of this is still ongoing. 

\paragraph{Intuitions on which formula works}
\begin{enumerate}
	\item When SGD and Adam yield similar fine-tuning results, we likely will not see a big difference across any of the kernel formulas, especially for smaller $K$.
	\item When Adam is better than SGD, we expect either SignGD or Asymmetric SignGD to work better than the standard SGD kernel formula.
	\item Asymmetric SignGD may perform worse than SignGD simply because solving the kernel regression with an asymmetric kernel is harder (see \Cref{sec:kernel_solvers}). 
	\item When fine-tuning involves more gradient steps (e.g., larger $K$ with fixed batch size), the Asymmetric SignGD kernel should do better than SignGD, because the SignGD kernel derivation only holds when the network is trained for very few steps. But this effect may be mitigated by the above issue with using an asymmetric kernel.
	\item The kernel can outperform fine-tuning for smaller $K$ because it is not as susceptible to noisy gradients as the fine-tuning optimization procedure would be. A noisy gradient can completely throw the trajectory off, but the kernel would just learn to down-weight that datapoint.
\end{enumerate}

\subsection{Kernel Solvers}\label{sec:kernel_solvers}
Once we compute the kernel, we need to solve the kernel regression problem. At this stage, it doesn't matter which formula or logit model was used. We can treat the train-train kernel as $K\times K$.\footnote{In the case of the individual logit model, we would repeat this process $C$ times independently. In the case of modeling across logits, we would solve this problem once but learn $\alpha\in\sR^{CK}$.}
We need to train the kernel regression coefficients. For a training set $\{(x_i,y_i)\}_{i=1}^K$, we want to learn $\alpha\in\sR^K$ such that 
$$\hat y_i = \sum_{j=1}^K \alpha_j \gK(x_i, x_j)$$

and we minimize $\ell(\hat{y}, y)$ for some loss function $\ell$. In other words, we want to model the output as a linear combination of the kernel function comparing the given datapoint to every training datapoint. We can train $\alpha$ using the train-train kernel and then check the validation and test performance of the kernel by using the train-validation and train-test kernels accordingly with the learned coefficients.

\paragraph{Choices for $\ell$} Since we have precomputed the kernel matrix, we can find $\alpha$ by solving a least squares problem directly. The other option is to choose $\ell$ as the logistic loss and then do gradient descent to find $\alpha$. We can also solve the kernel SVM problem, which was shown to be useful for NTK application to small datasets in \cite{arora2019harnessing}. We also try to perform $\ell_2$ regularization, where the coefficient is set proportional to the operator norm of the kernel to have a nonnegligible effect (this can result in a very large coefficient, like 10,000).

\paragraph{Adjusting for Initialization and Label Scaling} The NTK formulation relies on a Taylor expansion around the model's initialization. In all preceding NTK derivations, the model was randomly initialized, so its value (ie 0th order term in Taylor expansion) was 0 in expectation. In our case, we have a pre-trained model and we are adding a prompt. As such the model's output at initialization has some information and should not be ignored, so we should add the pre-trained model's output logit to the kernel's output. In the case where the label is unscaled, this will not make a huge difference, but as the label magnitude increases, it will be more and more important. We should scale the label and adjust for initialization to test the theory rigorously, but it may be the case that we don't find the correct label scaling to get the ideal result in practice. 

\paragraph{Asymmetric Kernel Solver}
We write how to solve the kernel regression problem with an asymmetric kernel here. This is an existing result, but in the context of NTK we might be able to make it a little bit stronger. Consider the augmented linear system:
$$
\begin{bmatrix} 0 & 0 & Y^\top & 0 \\ 0 & 0 & 0 & Y^\top \\ Y & 0 & I/\gamma & H \\ 0 & Y & H^\top & I/\gamma\end{bmatrix}\begin{bmatrix} b_1\\b_2 \\ \alpha \\ \beta\end{bmatrix} = \begin{bmatrix} 0 \\ 0 \\ 1 \\ 1 \end{bmatrix}
$$
where $H_{ij} = y_i\phi_s(x_i)^\top \phi_t(x_j) y_j$ with $\phi_s$ and $\phi_t$ as the two different feature maps and $y_i$ as the label for the $i$th example.
Define $\omega^*$ and $\nu^*$ as 
\begin{align*}
	\omega^* = \sum_i \beta_i^* y_i\phi_t(x_i) \\
	\nu^* = \sum_i \alpha_i^* y_i\phi_s(x_i)	
\end{align*}
Solving this system yields two discriminant functions:
\begin{align*}
	f_s(x) &= K(x,X)(\beta^*\odot Y) + b_1^* \\
	f_t(x) &= K(X,x)(\alpha^*\odot Y) + b_2^*	
\end{align*}

where $K(x_i,x_j) = \langle \phi_s(x_i), \phi_t(x_j)\rangle$.

We can thus create one discriminant function as $cf_s(x) + (1-c)f_t(x)$ where $c\in[0, 1]$ is some hyperparameter. When $\phi_s=\phi_t$, we see that $f_s=f_t$ and we reduce to the standard kernel problem (though with repeated equations).
We should only use $f_s$ as the predictor according to the theory.

\subsection{Linearized Model}
We can compare the model output to what the linearization would have given to get a predictive measure of how well fine-tuning can be described by the kernel regime. We need access to a pre-trained model and the corresponding fine-tuned model to do so. In the kernel regime, we expect that 
$$ f(\theta_{\text{FT}}) \approx f(\theta_{\text{PT}}) + \langle \nabla f(\theta_\text{PT}), \theta_{FT} - \theta_\text{PT}\rangle $$

\begin{table}[t]
\caption{Linearized Model vs. Standard Model. We compare the distance between the linearized model and the full model on the train data.}
\label{tab:linearized}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf Task}  &\multicolumn{1}{c}{\bf MSE (train)}
\\ \hline \\
SST-2 & xx \\
CR & xx \\
MPQA & xx \\
\end{tabular}
\end{center}
\end{table}





